Polyhedral Clinching Auctions and the Adwords Polytope

A central issue in applying auction theory in practice is the problem of dealing with budget-constrained agents. A desirable goal in practice is to design incentive compatible, individually rational, and Pareto optimal auctions while respecting the budget constraints. Achieving this goal is particularly challenging in the presence of nontrivial combinatorial constraints over the set of feasible allocations. Toward this goal and motivated by AdWords auctions, we present an auction for {\em polymatroidal} environments satisfying the above properties. Our auction employs a novel clinching technique with a clean geometric description and only needs an oracle access to the submodular function defining the polymatroid. As a result, this auction not only simplifies and generalizes all previous results, it applies to several new applications including AdWords Auctions, bandwidth markets, and video on demand. In particular, our characterization of the AdWords auction as polymatroidal constraints might be of independent interest. This allows us to design the first mechanism for Ad Auctions taking into account simultaneously budgets, multiple keywords and multiple slots. We show that it is impossible to extend this result to generic polyhedral constraints. This also implies an impossibility result for multi-unit auctions with decreasing marginal utilities in the presence of budget constraints.

==> budgets-adwords.tex <==
\section{Sponsored Search and the AdWords Polytope}\label{ad_words_polytope}

We describe the sponsored search setting and characterize the feasible
allocations in this setting as a polymatroid, which we call the AdWords
polytope. The present model generalizes the classical models of Edelman,
Ostrovsky and Schwarz \cite{edelman07sellingbillions} and Varian
\cite{Varian06positionauctions}, by adding multiple keywords. 

Consider $n$ advertisers and $m$ keywords. Each
advertiser $i$ is interested in a subset of the keywords $\Gamma(i) \subseteq
[m]$. For a keyword $k$, we denote by $\Gamma(k)$, the set of advertisers
interested in this keyword. With each keyword $k$, we associate
$\abs{\Gamma(k)}$ positions. Position $j$ for keyword $k$ has
click-through-rate $\alpha^k_j$ (possiby zero) in such a way that for each $k$,
$\alpha^k_1 \geq \alpha^k_2 \geq \hdots \geq \alpha^k_{\abs{\Gamma(k)}}$. 

Assuming that each keyword get a large amount of queries (for now let's assume
that a query matches only a single keyword, but as it will become clear later,
our model easily generalizes for allowing one query to match more than one
keyword), we see $\alpha^k_j$ as the sum of number of clicks that the $j$-th
position of keyword $k$ gets across all queries that match it. For now, let's
assume that the number of clicks a player gets in slot $j$ of keyword $k$
depends only on $j,k$ and not on the identity of the player. We come back to
this point later.

\subsection{Single keyword}

First, consider the setting with a single keyword and all advertisers
interested in it. Let the click-through-rates be $\alpha_1 \geq \hdots \geq
\alpha_n$. Assuming we have a large number of queries associated with it, an
allocation is to associate for each query an allocation of advertisers to
position slots. As the number of queries grow, this is equivalent to consider a
probability distribution over the allocations. An allocation $\pi$ maps each
player $i$ to a position $\pi(i)$. Therefore, an allocation vector $x$ is
feasible iff there is a probability distribution over allocations such that:
$$x_i = \E_{\pi}[\alpha_{\pi(i)}]$$
Feldman et al \cite{feldman08} relate the problem of deciding if a vector $x$ is
feasible to a classical problem in scheduling theory - scheduling in related
machines with preemptions ($Q \vert pmtn \vert C_{\max}$ \cite{graham}). What
follows a re-statement of their characterization in a format that makes it
clear it is a polymatroidal environment.

\begin{lemma}[Feldman et al \cite{feldman08}]\label{single-keyword-lemma}
 An allocation vector $x$ is feasible iff for each $S$, $x(S) \leq
\sum_{j=1}^{\abs{S}} \alpha_j$, where $x(S) = \sum_{i \in S} x_i$ for each set
$S \subseteq [n]$.
\end{lemma}

Notice that $f_k(S) = \sum_{j=1}^{\abs{S}} \alpha^k_j$ is a submodular
function, so the set of feasible allocations for the single-keyword setting is
a polymatroid.

\subsection{Multiple keywords}

For the multiple-keyword setting, we say that an allocation vector $x$ is
feasible if we can write $x_i = \sum_{k \in \Gamma(i)} x_i^k$ in such a way
that the vector $(x^k_i)_{i \in \Gamma(k)}$ is feasible for keyword $k$, i.e.,
$x^k(S) \leq f_k(S)$ for every $S \subseteq \Gamma(k)$.

The fact that this allocation set is a polymatroid is a direct consequence of
the following generalized version of Hall's Theorem :

\begin{theorem}
 Given a bipartite graph $([n] \cap [m], E)$, $\Gamma(\cdot)$ its neighborhood
map, $m$ submodular functions $f_1, \hdots, f_m$ and the polymatroids defined
by them $P_1, \hdots, P_m$, then the set:
$$P^* = \{x \in \R^n_+; x_i = \sum_{j \in \Gamma(i)} x_i^j \text{  and  } x^j
\in P_j \} $$
is a polymatroid defined by the function $f^*(S) = \sum_j f_j(S \cap
\Gamma(j))$.
\end{theorem}

\begin{proof}
 If $x \in P^*$, then clearly $x(S) \leq f^*(S), \forall S$. Now, for the
other direction, suppose the vector $\hat{x}$ is such that $\hat{x}(S) \leq
f^*(S), \forall S$. We need to show that there exist $x_i^j$ such that:
\begin{equation}\label{hall-primal}
\begin{aligned}
& \sum_{j \in \Gamma(i)} x_i^j = \hat{x}_i, & \forall i \\
& \sum_{i \in S} x_i^j \leq f_j(S), &\forall S \subseteq \Gamma(j) \\
& x_i^j \geq 0, & \forall i,j
\end{aligned}
\end{equation}
Showing that the program (\ref{hall-primal}) is feasible is equivalent to
showing that the solution of the dual program (\ref{hall-dual}) is bounded,
which is the same as all the feasible points having non-negative objective:
\begin{equation}\label{hall-dual}
\begin{aligned}
& \min \sum_i y_i \hat{x}_i + \sum_{j, S \subseteq \Gamma(j)} z_S^j f_j(S)
\qquad \text{s.t.} \\
& y_i + \sum_{S \subseteq \Gamma(j), S \ni i} z_S^j \geq 0, & \forall j \in
\Gamma(i) \\
& z_S^j \geq 0
\end{aligned}
\end{equation}
This is equivalent to proving that for all $z_S^j \geq 0$, the following is true:
\begin{equation}\label{goal-lemma-3}
-\sum_i \hat{x}_i \left( \min_{j \in \Gamma(i)} \sum_{S; i\in S \subseteq
\Gamma(j) } z_S^j  \right) + \sum_{j, S \subseteq  \Gamma(j)}  f_j(S) z_S^j
\geq 0
\end{equation}

To show this fact, define $\chi(i) = \min_{j \in \Gamma(i)} \sum_{S; i\in S
\subseteq \Gamma(j)} z_S^j $. Wlog we can assume that $\chi(1) \geq \chi(2) 
\geq \hdots \chi(n)$. Given that, we can rewrite:
$$\sum_i \hat{x}_i \chi(i) = \sum_i (\chi(i) - \chi(i+1)) \sum_{t \leq i}
\hat{x}_t \leq \sum_i (\chi(i) - \chi(i+1)) \sum_j f_j(\{1..i\} \cap \Gamma(j))
$$
To show (\ref{goal-lemma-3}), I'll show that for each $j$:
$$\sum_i (\chi(i) - \chi(i+1)) f_j(\{1..i\} \cap \Gamma(j)) \leq  \sum_{S
\subseteq  \Gamma(j)}  f_j(S) z_S^j$$
We do so by rewritting the equation above in terms of the marginals:
$$\sum_i (\chi(i) - \chi(i+1)) \sum_{t \in \{1..i\} \cap \Gamma(j) }
f_j(t \vert \{1..t-1\} \cap \Gamma(j)) \leq \sum_{S
\subseteq  \Gamma(j)}   z_S^j \sum_{t \in S} f_j(t \vert \{1..t-1\} \cap S)$$
where $f(i \vert S) = f(S \cup i) - f(S)$.
Now, we invoke submodularity to see that for $S \subseteq \Gamma(j)$, $f_j(t
\vert \{1..t-1\} \cap S) \geq f_j(t \vert \{1..t-1\} \cap \Gamma(j))$. Now,
after applying this inequality, compare the coefficients of $f_j(t \vert
\{1..t-1\} \cap \Gamma(j))$ in each of the sides. In the left side, the
coefficient is $\chi(t)$ and for the right side, the coefficient is $\sum_{S
\subseteq \Gamma(j), t \in S} z_S^j$. Now, by the definition of $\chi$,
$\chi(t) \leq \sum_{S \subseteq \Gamma(j), t \in S} z_S^j$
\end{proof}



\subsection{Quality factors}

More generally, we would like to consider the click-through-rate of a slot
depending also on the player allocated in that slot. Let $\alpha^k_{j,i}$ be the
click-through-rate of position $j$ of keyword $j$ when player $i$ is placed
there. Traditionally, we consider click-through-rates in produce form, i.e.,
$\alpha^k_{j,i} = \alpha^k_j \cdot \gamma^k_i$ where $\gamma^k_i$ is called
\emph{quality factor}. In a similar way, one can define a polytope of feasible
allocations, but in general it won't be a polymatroid.

If the quality factors are uniform among all queries,
i.e., $\gamma^k_i = \gamma_i$, the the set of feasible allocations is given by
$P^*_\gamma = \{x; (\frac{x_i}{\gamma_i})_i \in P^*\}$ where $P^*$ is the
polymatroid defined in the previous subsection as a function of $\alpha^k_j$.
It is a scaled polymatroid, for which a variant of the auction in the following
section works. 
